Model Checking Epistemic Halpern-Shoham Logic Extended with Regular Expressions

The Epistemic Halpern-Shoham logic (EHS) is a temporal-epistemic logic that combines the interval operators of the Halpern-Shoham logic with epistemic modalities. The semantics of EHS is based on interpreted systems whose labelling function is defined on the endpoints of intervals. We show that this definition can be generalised by allowing the labelling function to be based on the whole interval by means of regular expressions. We prove that all the positive results known for EHS, notably the attractive complexity of its model checking problem for some of its fragments, still hold for its generalisation. We also propose the new logic EHSre which operates on standard Kripke structures and has expressive power equivalent to that of EHS with regular expressions. We compare the expressive power of EHSre with standard temporal logics.

==> logics.tex <==
\section{Languages of Specification}
The aim of this section is to define the Epistemic Halpern--Shoham logic, \ehs{}, that is a mix of epistemic modal logic and Halpern--Shoham logic. We first focus on the adaptation of the concept of knowledge to interval-based interpreted systems. To this end, we define a simpler logic called \eit{}.

\subsection{Knowledge on intervals}
The Epistemic Interval Temporal Logic (\eit{}) syntax is exactly the same as the syntax of epistemic modal logic:
\[
\varphi ::= p | \neg \varphi | \varphi \wedge \varphi | K_i \varphi
\]
where $p$ is a propositional variable and $i$ is an agent. Boolean connectives $\vee, \Rightarrow, \Leftrightarrow$ are introduced in the standard way.

The truth values of formulae of EIL logic in a interval-based interpreted structure $\str{M}$ and an interval ${\cal I}$ are determined by the following semantic rules:
\begin{enumerate}
\item For all $v \in {\cal V}ar$, we have $\str{M}, {\cal I} \models v$ iff $v \in \gamma({\cal I})$.
\item $\str{M}, {\cal I} \models \neg \varphi$ iff $\str{M},{\cal I} \not \models \varphi$.
\item $\str{M}, {\cal I} \models \varphi_1 \wedge \varphi_2$ iff $\str{M}, {\cal I}  \models \varphi_1$ and $\str{M}, {\cal I}  \models \varphi_2$.
\item $\str{M}, {\cal I} \models K_i \varphi$, where $i$ is an agent, iff for all ${\cal I'} \sim_i {\cal I}$ we have $\str{M}, {\cal I'}  \models \varphi$.
\end{enumerate}

The above definition is almost the same as the semantics of epistemic modal logic. The only essential difference that we need to discuss is the definition of relation $\sim_i$. Roughly speaking, we define it in a way such that an agent cannot distinguish between two intervals in they have the same length and the consecutive states are indistinguishable for him. This seams to be close to the standard definitions \nb{jm: some references?}.

Formally, we define $\sim_i$ on states first. We put $s \sim_i s'$ if and only if $l_i(s)=l_i(s')$, i.e., the local states of $i$th agent are the same in both states. We define $\sim_i$ on intervals as $s_1, \dots s_k\sim_i {s'}_1, \dots, {s'}_l$ iff $k=l$ and for all $j\leq k$, $l_i(s_j)=l_i({s'}_j)$. 

The logic \eit{} is quite simple. The modality $K_i$ can be read as, roughly speaking, ``in all $\sim_i$ equivalent intervals it holds that''.

\begin{example}Consider a Kripke structure containing states $s$ and $t$ such that the pair $(s, t)$ is the only one labelled by a propositional variable $p$, an agent $1$ that cannot distinguish any states, i.e. $u \sim_1 u'$ for all states $u, u'$, and a formula $\neg K_1 \neg p$. This formula is true in an interval of length $n$ if and only if there is a path from $s$ to $t$ of length $n$.
\end{example}

\subsection{Common knowledge}
Now we extend the logic \eit{} by the concept of common knowledge \nb{jm: references needed, or some other kind of glue}. 

The logic \eitp{} extends \eit{} by operator $C_G$, read as ``it is a common knowledge in $G$ that''. Formally, the syntax of \eitp{} is defined as
\[
\varphi ::= p | \neg \varphi | \varphi \wedge \varphi | K_i \varphi | C_G \varphi
\]
where $p$ is a propositional variable, $i$ is an agent and $G$ is a set of agents.

Let $E_G\varphi$ stand for $\bigwedge_{i \in G} K_i \varphi$. We define $E^i_G$ as $E_G^0 \varphi = \varphi$ and $E_G^{n+1} \varphi =E_G E_G^n \varphi$. The semantics of \eitp{} extends the semantic of \eit{} by the following rule:
\begin{enumerate}
\item[5.] $\str{M}, {\cal I} \models C_G \varphi$, where $G$ is a group of agents, iff for all $n\in N$ we have $\str{M}, {\cal I}  \models E_G^n \varphi$.
\end{enumerate}

\subsection{Epistemic Halpern--Shoham Logic}
The logic \eitp{} contains no modal operators other than $K_i$. In this section, we fix it by extending the logic by Halpern--Shoham modalities.

The modal operators of the Halpern--Shoham logic comes from so-called Allen's relations between intervals, defined by Allen in '83 \cite{Al83}. 
Six of these relations, $R_A$ (a.k.a. ``after``, ``meets'') , $R_B$ (a.k.a. ``begins'', ``starts''), $R_D$ (a.k.a. ``during''), $R_E$ (a.k.a. ``ends''), $R_O$ (a.k.a. ''overlaps'') and $R_L$ (a.k.a. ``later'') are defined in Fig. \ref{f:allens}. For each of these relations $R_X$, we also define the inverted relation $R_{\bar{X}}={R_X}^{-1}$.

\begin{figure}[!ht]
\stikz{allen.tikz}
\caption{Basic Allen's relations}\label{f:allens}
\end{figure}

Formally, the syntax of Epistemic Halpern--Shoham Logic (\ehs{}) is defined as 

\[\begin{array}{rcl}
\varphi &::=& p | \neg \varphi | \varphi \wedge \varphi | K_i \varphi | C_G \varphi |\\
& &\langle A \rangle \varphi | \langle \bar{A} \rangle \varphi|
\langle B \rangle \varphi| \langle \bar{B} \rangle \varphi|
\langle D \rangle \varphi| \langle \bar{D} \rangle \varphi|\\
& &\langle E \rangle \varphi| \langle \bar{E} \rangle \varphi|
\langle L \rangle \varphi| \langle \bar{L} \rangle \varphi|
\langle O \rangle \varphi| \langle \bar{O} \rangle \varphi 
\end{array}
\]
where $p$ is a propositional variable, $i$ is an agent and $G$ is a set of agents. Boolean connectives $\vee, \Rightarrow, \Leftrightarrow$ are introduced in the standard way. 

We abbreviate $\neg \naw{X} \neg \varphi$ by $[X]\varphi$. By $X_1X_2\dots X_n$ \emph{fragment} of \ehs{} logic we define the fragment of \ehs{} in which only modal operators allowed are $K_i$, $C_G$, and $\naw{X_1}$, \dots, $\naw{X_n}$. 

The semantics of \ehs{} extends the semantics of EIL by the following semantics rule:
\begin{enumerate}
\item[6.] $\str{M}, {\cal I} \models \naw{X} \varphi$ for, where $X$ is any Allen relation, iff there exists an interval ${\cal I'}$ such that ${\cal I} R_X {\cal I'}$ and  $\str{M}, {\cal I'} \models \varphi$.
\end{enumerate}

We often use operator $[G]$ defined as
\[
[G] \varphi = \varphi \bigwedge_{X\in\{A,B,D,E,L,O\}} ([X]\varphi \wedge [\bar{X}] \varphi)
\]
which can be read as ``in all reachable intervals'', and its existential version $\naw{G}$ that can be read as ``there is a reachable interval such that''. We define the abbreviation $\naw{X}^i$ recursively as $\naw{X}^0 \varphi=\varphi$, $\naw{X}^{i+1} \varphi=\naw{X}(\naw{X}^i \varphi)$.

\begin{example}
Consider following formulae.
\[
 \naw{G} (\naw{B}s\wedge \naw{E}t \wedge ([D] ([B] \bot \Rightarrow K_1 safe)) )
\]
It states that there is a way for agent $1$ to get from a world satisfying  $s$ to a world satisfying $t$ using only safe states (notice that $[B] \bot$ is satisfied only in point intervals).

\[
 [G](\naw{B} request \wedge \naw{B}^{10} \Rightarrow (\naw{D} fulfill \vee \naw{E} fulfill))
\]
It states that each request (modelled as a point interval labelled by $request$), is fulfilled (modelled as a point interval labelled by $fulfill$) after at most $10$ steps.


\[
 [G](printing \Rightarrow \naw{\dei} printing\_request\_processing)
\]
It states that if printer is printing, then it is in the middle of processing sone printing request.

\nb{jm: it is a stub only}. More examples are in Section \ref{s:examples}.
\end{example}

A reader that is already familiar with the Halpern-Shoham logic should notice here that some choices that are typically discussed before the definition of the semantics of the Halpern--Shoham logic follow from our definition of models. In particular, the considered order are tree-like, but not necessarily linear, and we allow for point interval, i.e. intervals that consists of one state only.

The logic \ehs{} is quite expressive. For example, it is possible to write a formula that is true if and only if a model contain an interval that represents a successful run of a Turing machine, even using only one operator, namely $\naw{D}$ \cite{MM11}. More examples of interesting properties that can be expressed in this logic are in Section \ref{s:examples}.
